LLM as a Scorer: The Impact of Output Order on Dialogue Evaluation

This research investigates the effect of prompt design on dialogue evaluation using large language models (LLMs). While LLMs are increasingly used for scoring various inputs, creating effective prompts for dialogue evaluation remains challenging due to model sensitivity and subjectivity in dialogue assessments. Our study experimented with different prompt structures, altering the sequence of output instructions and including explanatory reasons. We found that the order of presenting reasons and scores significantly influences LLMs' scoring, with a "reason-first" approach yielding more comprehensive evaluations. This insight is crucial for enhancing the accuracy and consistency of LLM-based evaluations.

==> tables/fig_main.tex <==
\begin{figure}
    \centering
    \includegraphics{AnonymousSubmission/data/scores.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

==> tables/fig_prompt.tex <==
\begin{figure*}[t]
\centering
\includegraphics[trim={0cm 0.75cm 0cm 2.7cm},clip,width=\linewidth]{data/fig_method.pdf}
\caption{The form of prompt for LLM scorer in conversation evaluation.}
\label{fig:method}
\end{figure*}

==> tables/fig_tease.tex <==
\begin{figure}[t]
\centering
\includegraphics[trim={2cm 0cm 7cm 0cm},clip,width=\linewidth]{data/fig_tease.pdf}
\caption{An example of impacts on a LLM scorer outputs, with merely swapping the order of output instructions. While the reasons are similar, the scores given are obviously different. (temp, fontsize too small)}
\label{fig:tease}
\end{figure}
